How to Fill the Optimum Set? Population Gradient Descent with Harmless Diversity

Although traditional optimization methods focus on finding a single optimal solution, most objective functions in modern machine learning problems, especially those in deep learning, often have multiple or infinite numbers of optima. Therefore, it is useful to consider the problem of finding a set of diverse points in the optimum set of an objective function. In this work, we frame this problem as a bi-level optimization problem of maximizing a diversity score inside the optimum set of the main loss function, and solve it with a simple population gradient descent framework that iteratively updates the points to maximize the diversity score in a fashion that does not hurt the optimization of the main loss. We demonstrate that our method can efficiently generate diverse solutions on a variety of applications, including text-to-image generation, text-to-mesh generation, molecular conformation generation and ensemble neural network training.

==> tex/old_notes.tex <==

\section{Main Method} 

Given a loss function $f(x)$, we want to find a set of particles $\{x_i\}$ in the argmin set of $f$ that are as diverse as possible. 
This can be framed into a lexico problem: 
$$
\max_{\{x_i\}} \Phi(\{x_i\}) ~~~~~s.t. ~~~~ x_i \in \argmin f. 
$$
where $\Phi(\{x_i\})$ is some measure of diversity. 
Equivalently, we can frame the problem into
$$
\max_{\{x_i\}} \Phi(\{x_i\}) ~~~~~s.t. ~~~~  \sum_{i=1}^m f(x_i) \leq m f^*, 
%x_i \in \argmin f. 
$$
where $f^* = \min_x f(x)$. Here it is important to use a single constraint of $\sum_{i=1}^m f(x_i) \leq m f^*$, because it allows us to increase one objective in exchange of decreasing another. 
 It is better than enforcing all the constraints $f(x_i) \leq f^*$. 

%We consider iterative updates of form 
Assume we plan to update $x_i$ to $x_i'$ and the goal is to derive the optimal choice of $x_i'$. 

The choice of $x_i'$ should ensure that 1) $\sum_{i=1}^m f(x_i) $ decreases, and 2) $\Phi$ is minimized. 

Note that here we do not require that every $f(x_i)$ decrease. It is sufficient and important to ensure 
 $\sum_{i=1}^m f(x_i) \leq m f^*$ decrease, because it allows us to increase one objective in exchange of decreasing another (the particles can exchange loss with either other for a better global loss). 
% It is better than enforcing all the constraints $f(x_i) \leq f^*$. 


%$$x_i' \gets x_i  - \epsilon v_i,$$
%such that $\sum_{i=1}^m f(x_i)$ decreases. Note that 
Assume $f$ is $1/\mu$-smooth, that is, $\norm{\dd^2 f(x)}\leq 1/\mu$ for any $x$. We have 
\bb 
\sum_{i=1}^m f(x_i') 
%& = \sum_{i=1}^m f(x_i - \epsilon v_i) \\
& \leq  \sum_{i=1}^m \bigg ( f(x_i) + \dd f(x_i)\tt  (x_i' -x_i) + \frac{1}{2\mu} \norm{x_i' - x_i}^2 \bigg)\\
& = \sum_{i=1}^m \bigg ( f(x_i) +  \frac{1}{2\mu} \norm{x_i' - x_i + \mu \dd f(x_i)}^2  - \frac{\mu}{2} \norm{\dd f(x_i)}^2 \bigg ) \\
& = \sum_{i=1}^m  f(x_i) +  \frac{1}{2\mu}\bigg ( \sum_{i=1}^m \norm{x_i' - y_i}^2 - \epsilon_0^2 \bigg).
%\norm{x_i' - x_i + \mu \dd f(x_i)}^2  - \frac{\mu}{2} \norm{\dd f(x_i)}^2 \bigg ). 
\ee
where we define $$y_i = x_i - \mu \dd f(x_i),~~~~~~~~ \epsilon_0^2 = \sum_{i=1}^m {\mu^2}  \norm{\dd f(x_i)}^2.$$
To make sure that $\sum_i f(x_i') \leq \sum_i f(x_i)$, we hope to enforce that 
$$
\sum_{i=1}^m   \norm{x_i' - y_i}^2  \leq  \epsilon^2,
$$
where 
$$
\epsilon = \eta \epsilon_0,
$$
and $\eta \in (0,1)$ is a coefficient that controls the repulsive magnitude. 

Therefore, at each iteration, we may want to decide $\{x_i'\}$ by 
$$
\max_{v_i} \Phi(\{x'_i\}) ~~~~s.t.~~~~   \sum_{i=1}^m   \norm{x_i' - y_i}^2  \leq  \epsilon^2.
%\norm{x_i' - x_i - \mu \dd f(x_i)}^2  \leq  \frac{\mu^2}{2} \norm{\dd f(x_i)}^2 
$$
Now let us consider the special case when  $\Phi$ is the variance: 
$$
\Phi(\vv x) = \sum_{i,j=1}^m \norm{x_i - x_j}^2. 
$$
%We have the KKT condition: 
The lagrangian form of the optimization is: 
$$
 \max_{v_i} \min_{\lambda \geq 0} \sum_{i,j=1}^m  \norm{x_i '- x_j'}^2  - \lambda \left ( \sum_{i=1}^m   \norm{x_i' - y_i}^2  -  \epsilon^2 \right). 
$$
Taking derivative w.r.t. $x_i'$ gives the following
KKT condition: 
$$
\sum_{j=1}^m  (x_i' - x_j') + \lambda (x_i' - y_i) = 0,~~~~\forall i\in[m]. 
$$
%Gives
$$
 n x_i' + n \bar x' + \lambda (x_i - y_i) = 0.
$$
$$
x_i' = \frac{\lambda y_i   - n \bar x'}{\lambda - n} =  \frac{(\lambda-n) y_i + n y_i   - n \bar x'}{\lambda - n} 
= y_i + \frac{n}{\lambda -n} (y_i - \bar x') = y_i +  \alpha (y_i - \bar x'). 
$$
where  we 
take $\bar x' = \sum_{i=1}^m x_i' /m $ and 
let $\alpha = n/(\lambda -n)$. % We have $x_i' =  y_i + \alpha (y_i - \bar x')$.
Taking average on both sides: %them together: 
$$
 \bar x'=  (1+\alpha )\bar y -  \alpha \bar x',
$$
where $\bar y = \sum_{i=1}^m y_i/m$. 
This gives $\bar x' = \bar y$. 
So 
$$
x_i' = y_i + \alpha (y_i - \bar y). 
$$
Plugging this back to the original problem: 
$$
\min_{\alpha} - \sum_{i=1}^m (1+\alpha)^2\norm{y_i - \bar y} ^2 ~~~~~s.t.~~~~ \sum_{i=1}^m \alpha^2 \norm{y_i - \bar y} \leq \epsilon^2. 
$$
Equivalent to 
$$
\max_\alpha   (1+\alpha)^2 ~~~~~s.t.~~~~~\alpha^2 \leq \frac{\epsilon^2}{\sum_{i=1}^m \norm{y_i - \bar y}^2}.
$$
This gives that 
$$
\alpha^* =  \frac{\epsilon}{\sqrt{\sum_{i=1}^m \norm{y_i - \bar y}^2}}.
$$
Hence 
$$
x_i' = y_i +  \alpha^* (y_i -\bar y),~~~~~~~~~~\alpha^* =  \frac{\sqrt{\sum_{i=1}^m {\mu^2} \norm{\dd f(x_i)}^2}}{\sqrt{\sum_{i=1}^m \norm{y_i - \bar y}^2}} 
= \frac{\sqrt{\sum_{i=1}^m \norm{y_i - x_i}^2}}{\sqrt{\sum_{i=1}^m \norm{y_i - \bar y}^2}} $$

\begin{tcolorbox}
\textbf{Goal}: Find a set of diversified local minima of a loss $f(x)$.  \\
\textbf{Hyper-parameters}:  step size $\mu >0$, a repulsive coefficient $\eta$.  
At the $t$-th iteration: %Take 
\bb 
& y_{i}^t = x_i^t - \mu \dd f(x_i^t),  \\
&\bar y^t = \frac{1}{m} \sum_{i=1}^m y_i\\
&\alpha^*_t =  \frac{\sqrt{\sum_{i=1}^m \norm{y_i - x_i}^2}}{\sqrt{\sum_{i=1}^m \norm{y_i - \bar y}^2}} \\
&x_{i}^{t+1} \gets y_i^t +  \eta \alpha_t^* (y_i^t - \bar y^t)
\ee 
\end{tcolorbox} 

\iffalse
Test code here: \url{https://colab.research.google.com/drive/1QcWQeN0bvoymLb7UbAj-80EGQay-mXuC?usp=sharing} 
\fi

\subsection{General Diversity measure} 
Consider
$$
\max_{\vv x'} 
\Phi(\vv x') ~~~s.t.~~~~\sum_{i=1}^m \norm{x_i' - y_i}^2 \leq \epsilon^2.
$$
Apply Taylor approximation on $\Phi$. 
Let $g_i = \partial_i \Phi(\vv y)$.
We have 
$$
\max \sum_i g_i \tt (x_i'-y_i) ~~~s.t.~~~~\sum_{i=1}^m \norm{x_i' - y_i}^2 \leq \epsilon^2.
$$
So it is 
$$
\max \sum_i g_i \tt \delta_i ~~~s.t.~~~~\sum_{i=1}^m \norm{\delta_i}^2 \leq \epsilon^2.
$$

$$
\max \sum_i g_i \tt \delta_i - \lambda (\sum_{i=1}^m \norm{\delta_i}^2 - \epsilon^2).
$$
$$
g_i - \lambda \delta_i = 0.  
$$
Plug this back: 
$$
\max \sum_i\alpha \norm{ g_i }^2 ~~~s.t.~~~ \sum_i \alpha^2 \norm{g_i}^2 \leq \epsilon^2.
$$
This gives 
$$
\alpha = \frac{\epsilon}{\sqrt{\sum_i \norm{g_i}^2}}
$$
So the update is 
$$
x_i' = x_i -\mu \dd f(x_i) + \alpha g_i. 
$$
With 
$$
\alpha = 
\frac{\sqrt{\sum_{i=1}^m {\mu^2} \norm{\dd f(x_i)}^2}}{\sqrt{\sum_{i=1}^m \norm{g_i}^2}} 
= \frac{\sqrt{\sum_{i=1}^m \norm{y_i - x_i}^2}}{\sqrt{\sum_{i=1}^m \norm{g_i}^2}} 
$$

Assume 
$$
\Phi(\vv x) = \sum_{ij} \phi(\norm{x_i- x_j}^2). 
$$
Let $w_{ij} = \phi'(\norm{x_i-x_j}^2)$
We have 
$$
\partial_i \Phi(\vv x) = \sum_{j\neq i} 
2 w_{ij} (x_i - x_j) 
= (\sum_{j} w_{ij}) x_i - \sum_j w_{ij} x_j. 
$$

\subsection{Extension with Momentum}
%Adding a 
Let $v_i$ be  a momentum associated with $x_i$. Define a Hamiltonian:
$$
H(\vv x,\vv v) = \sum_{i=1}^m f(x_i) +
\frac{1}{2} \norm{v_i}^2 -
 \frac{1}{2}\eta \norm{v_i - \bar v}^2 ,~~~~\bar v = \sum_i v_i/m. 
$$
Taking standard gradient on $\vv x$ and $\vv v$: 
\bb 
&\dot x_i = - \dd f(x_i) \\
&\dot v_i = - v_i + \eta (1-\frac{1}{m})( v_i - \bar v).
\ee 
Adding a skew-symmetric component: 
\bb 
&\dot x_i = - \dd f(x_i)  - v_i  \\
&\dot v_i = - v_i + (1-\frac{1}{m})( v_i - \bar v) + \beta \dd f(x_i).
\ee 
\red{Tested: Does not seem to be as good as the diversified gradient version.}


\subsection{Adding Momentum: V2}
Assume we perform the following momentum like update: 
\bb 
& v_i' = v_i - \delta_i \\
& x_i' = x_i + v_i' 
\ee 
and we need to decide the optimal $\delta_i$. 
Consider Hamiltonian 
$$H(\vv x,\vv v) = \sum_{i=1}^m f(x_i) +
\frac{1}{2}\beta \norm{v_i}^2 $$

So 
\bb
H(\vv x',\vv v') - H(\vv x, \vv v) 
& \leq 
\sum_{i=1}^m  \dd f(x_i)\tt (x'_i-x_i) + \frac{1}{2\mu} \norm{x_i' - x_i}^2 
+ \frac{1}{2} \beta\norm{v_i'}^2 - \frac{1}{2} \beta \norm{v_i}^2 \\ 
& =\frac{1}{2\mu} \bigg (\sum_{i=1}^m \norm{x_i' - y_i}^2  - \epsilon_0^2 \bigg  ) + \frac{1}{2}\beta ( \norm{v_i'} ^2 - \norm{v_i}^2 )\ant{$y_i = x_i - \mu \dd f(x_i)$, $\epsilon_0^2 = \sum_i \norm{\mu\dd f(x_i)}^2$}\\
%& =\frac{1}{2\mu} \bigg (\sum_{i=1}^m \norm{x_i + v_i - \delta_i - y_i}^2  - \epsilon_0^2 \bigg  ) + \frac{1}{2} \beta( \norm{v_i - \delta_i} ^2 - \norm{v_i}^2)
& =\frac{1}{2\mu} \bigg (\sum_{i=1}^m \norm{x_i' - y_i}^2  - \epsilon_0^2    + \mu\beta \norm{x_i' -x_i} ^2 - \mu\beta \norm{v_i}^2 \bigg ) \\
& = \frac{1}{2\mu} \bigg (\sum_{i=1}^m 
(1+\mu\beta) \norm{x_i' - z_i}^2 
+ \left[  
(1+\mu\beta) \norm{x_i - z_i}^2 
-  \mu \beta \norm{v_i}^2 
\right]
\bigg)\\
& = \frac{(1+\mu\beta)}{2\mu} \bigg (\sum_{i=1}^m 
 \norm{x_i' - z_i}^2 
- \xi_0^2
\bigg)
\ee 
where we define 
$$
z_i = \frac{1}{1+\mu\beta} (y_i + \mu\beta x_i) 
= \frac{1}{1+\mu\beta} (x_i - \mu \dd f(x_i) + \mu\beta x_i) 
 = x_i - \frac{\mu}{1+\mu\beta} \dd f(x_i) = x_i - \tilde \mu \dd f(x_i), 
$$
with $\tilde \mu =  \frac{\mu}{1+\mu\beta} $.  
\bb 
\xi_0^2
& =\sum_{i=1}^m \left[   \frac{\mu \beta}{1+\mu\beta} \norm{v_i}^2 - \norm{x_i - z_i}^2 \right]\\
& =\sum_{i=1}^m \left[   \tilde \mu \beta \norm{v_i}^2 - \norm{\tilde \mu \dd f(x_i)}^2 \right]\\
\ee 
%Define $z_i =x_i + v_i - y_i= v_i + \mu \dd f(x_i)$. 
Therefore, we may hope 
$$
% =%\frac{1}{2\mu} 
%\bigg (
\sum_{i=1}^m \norm{x_i' - z_i}^2 \leq \xi^2 \defeq \eta^2 \xi_0^2. 
% + \mu \beta \norm{x'_i - x_i} ^2 \leq  \eta (\mu \beta \norm{v_i}^2   + \epsilon_0^2)  \defeq \xi^2,
$$
where $\eta \in(0,1)$. 
In the variance case, we want to solve: 
$$
\max_{\delta} \sum_{ij} \norm{x_i'-  x_j'}^2 ~~~~s.t.~~~~ 
\sum_{i=1}^m \norm{x_i' - z_i}^2 \leq \xi^2 \defeq \eta \xi_0^2. 
%\sum_{i=1}^m \norm{x_i' - y_i}^2 + \mu \beta \norm{x'_i - x_i} ^2 \leq \xi^2.
$$

The solution is 
$$
x_i' = z_i +  \alpha^* (z_i -\bar z). 
$$
$$
\alpha^* =  \frac{\eta \xi_0}{\sqrt{\sum_{i=1}^m \norm{z_i - \bar z}^2}} 
= \eta \frac{\sqrt{\sum_{i=1}^m   \tilde \mu \beta \norm{v_i}^2 - \norm{\tilde \mu \dd f(x_i)}^2 }}{\sqrt{\sum_{i=1}^m \norm{z_i - \bar z}^2}}. 
$$

\begin{lem}
$$
\norm{x-a}^2 + \beta \norm{x-b}^2 =
(1+\beta)\norm{x- \frac{a+\beta b}{1+\beta}}^2 + 
\norm{a}^2 + \norm{b}^2 - (1+\beta) \norm{ \frac{a+\beta b}{1+\beta}}^2.
$$
\end{lem}

